Sparse Coding by Spiking Neural Networks: Convergence Theory and Computational Results

In a spiking neural network (SNN), individual neurons operate autonomously and only communicate with other neurons sparingly and asynchronously via spike signals. These characteristics render a massively parallel hardware implementation of SNN a potentially powerful computer, albeit a non von Neumann one. But can one guarantee that a SNN computer solves some important problems reliably? In this paper, we formulate a mathematical model of one SNN that can be configured for a sparse coding problem for feature extraction. With a moderate but well-defined assumption, we prove that the SNN indeed solves sparse coding. To the best of our knowledge, this is the first rigorous result of this kind.

==> SupportDoc2/abstract.tex <==


\begin{abstract}
This is really a working note on the evolving work since a long discussion among the authors
during which various ideas were explored in the formulation of spike rates from somebasic governing 
equations. These equations involve the soma current $\curr_i(t)$ of a neuron (the $i$-th one),  
the building up of potential $\poten_i(t)$ 
that leads to a spike at a certain time $\spike(t-t_{i,j})$, and the
exponential decaying influence to associated soma currents due to such a spikes.

In particular, this note uses one specific formulation of average soma current, $\avgcurr_i(t)$ and 
spike rate $\spikerate_i(t)$ and show that they are related by a differential equation. Under
moderate assumptions, they converge to a limit that corresponds to a fixed point of a related
LCA equation. In particular, when the nerons are connected appropirately, the spiking neural network
can be used to solve various problems including LASSO. 
\end{abstract}



==> SupportDoc2/authors.tex <==

\title{A Formulation of Locally Competitive Algorithm \\
by Spiking Neural Networks}

\author{Anonymous for blinded review}
\affil{Anonymous Institution}





==> SupportDoc2/lasso_macros.tex <==


\newcommand{\signature}{
\VS
Sincerely,\\
Ping Tak Peter Tang\\
Corresponding Author
}

\newcommand{\myfig}[5]{
\framebox[\textwidth]{
\epsfig{width=#2,height=#3,file=#1}
}
\caption{#4}\label{figure:#5}}

\newcommand{\PlaceHolder}[1]{
\framebox[0.9\textwidth]{
\parbox{0.4\textwidth}{
\begin{center}
{#1}
\end{center}}
}}

%\newcommand{\myfig}[4]{
%\framebox[6in]{
%\includegraphics{#1.#2}}
%\caption{#4}\label{figure:#3}}



\newtheorem{mydef}{Definition}
\newtheorem{mythm}{Theorem}
\newtheorem{myalgo}{Algorithm}
\newtheorem{mylemma}{Lemma}
\newtheorem{mycor}{Corollary}
\newtheorem*{myproof}{Proof}


\newcommand{\placeholder}{{\small\bf PLACE HOLDER}}

\newcommand{\NI}{\noindent}
\newcommand{\VS}{{\vspace*{0.1in}\NI}}


\newcommand{\reals}{\mathbb{R}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\realpart}{\operatorname{Re}}
\newcommand{\suchthat}{\;\mid\;}
\newcommand{\equivto}{\Leftrightarrow}



\newcommand{\Bnorm}[1]{\| {#1} \|_B}
\newcommand{\Enorm}[1]{\| {#1} \|_2}
\newcommand{\Enormsq}[1]{\| {#1} \|_2^2}
\newcommand{\Onenorm}[1]{\| {#1} \|_1}
\newcommand{\inverse}[1]{{#1}^{-1}}
\newcommand{\transpose}[1]{{#1}^{\rm t}}
\newcommand{\dist}[2]{\mathrm{dist}({#1},{#2})}
\newcommand{\ssup}[2]{{#1}^{(#2)}}
\newcommand{\start}[1]{\ssup{#1}{0}}



\newcommand{\vv}[1]{\mathbf{#1}}
\newcommand{\vd}[1]{\dot{\mathbf{#1}}}
\newcommand{\vva}{\vv{a}}
\newcommand{\vvb}{\vv{b}}
\newcommand{\vve}{\vv{e}}
\newcommand{\vvf}{\vv{f}}
\newcommand{\vvg}{\vv{g}}
\newcommand{\vvq}{\vv{q}}
\newcommand{\vvm}{\vv{m}}
\newcommand{\vvs}{\vv{s}}
\newcommand{\vvu}{\vv{u}}
\newcommand{\vvv}{\vv{v}}
\newcommand{\vvw}{\vv{w}}
\newcommand{\vvx}{\vv{x}}
\newcommand{\vvy}{\vv{y}}
\newcommand{\vvz}{\vv{z}}
\newcommand{\vvzero}{\vv{0}}


\newcommand{\cc}[1]{{\cal #1}}
\newcommand{\ccA}{\cc{A}}
\newcommand{\ccB}{\cc{B}}
\newcommand{\ccC}{\cc{C}}
\newcommand{\ccD}{\cc{D}}
\newcommand{\ccE}{\cc{E}}
\newcommand{\ccF}{\cc{F}}
\newcommand{\ccI}{\cc{I}}
\newcommand{\ccL}{\cc{L}}
\newcommand{\ccM}{\cc{M}}
\newcommand{\ccS}{\cc{S}}
\newcommand{\ccX}{\cc{X}}



\newcommand{\vvastar}{\vva^*}
\newcommand{\vvustar}{\vvu^*}
\newcommand{\ustar}{u^*}
\newcommand{\astar}{a^*}

\newcommand{\thresfun}{T}
\newcommand{\thres}{\thresfun_\lambda}
\newcommand{\vvthres}{\vv{\thresfun}_\lambda}
\newcommand{\lyap}{\xi}

\newcommand{\vvphi}{{\boldsymbol\phi}}

\newcommand{\vvT}{\vv{T}}
\newcommand{\vvF}{\vv{F}}

\newcommand{\vdu}{\vd{u}}

\newcommand{\ustart}{\ssup{\vv{u}}{0}}
\newcommand{\vstart}{\ssup{\vv{v}}{0}}
\newcommand{\vvahat}{\hat{\vva}}
\newcommand{\vvuhat}{\hat{\vvu}}
\newcommand{\vvvhat}{\hat{\vvv}}



\newcommand{\flowlasso}[2]{\vv{A}({#1},{#2})}
\newcommand{\flowlca}[2]{\vv{U}({#1},{#2})}
\newcommand{\vdA}{\vd{A}}
\newcommand{\vdU}{\vd{U}}

\newcommand{\grad}{\nabla}
\newcommand{\sign}{\mathrm{sign}}


\newcommand{\fixedpts}{{\cal F}}
\newcommand{\criticalpts}{{\cal C}}
\newcommand{\fixedregion}{\hat{\fixedpts}}




\newcommand{\ctrans}[1]{{#1}^{*}}
\newcommand{\tendsto}{\rightarrow}
\newcommand{\Chi}{\Pi}
\newcommand{\diag}{{\rm diag}}
\newcommand{\rank}{{\rm rank}}
\newcommand{\spann}{{\rm span}}
\newcommand{\gap}{{\rm gap}}
\newcommand{\offdiag}{{\rm off}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\tmpa}{{\rm dummy}}
\newcommand{\tmpb}{{\rm dummy}}
\newcommand{\tmpc}{{\rm dummy}}
\newcommand{\tmpd}{{\rm dummy}}

\newcommand{\Deltop}{\xi}
\newcommand{\Delbot}{\zeta}
\newcommand{\Deldc}{\psi}
\newcommand{\Deltrans}[1]{
\left[
\begin{array}{c | c}
  \begin{array}{c}
  \iterate{\Deltop}{#1} \\ 
  \iterate{\Delbot}{#1}
  \end{array}
 & \iterate{\Deldc}{#1}
\end{array}
\right]
}
\newcommand{\Linv}[1]{\iterate{L^{-1}}{{#1}}}


\newcommand{\quadf}{\rho}
\newcommand{\quadfbdd}{\xi}
\newcommand{\reference}{{\rm ref}}
\newcommand{\mm}{m}
\newcommand{\mprime}{m'}
\newcommand{\pp}{p}
\newcommand{\gapfactor}{\gamma}
\newcommand{\lambdamin}{\lambda_{-}}
\newcommand{\lambdamax}{\lambda_{+}}
\newcommand{\lambint}{(\lambdamin,\lambdamax)}
\newcommand{\lambintc}{[\lambdamin,\lambdamax]}
%\newcommand{\lambnum}{{\mathbf{i}}}
\newcommand{\lambnum}{e}
\newcommand{\surM}{M}
\newcommand{\calI}{{\cal I}}
\newcommand{\calC}{{\cal C}}
\newcommand{\projector}{{X_\calI}\ctrans{X}_\calI B}
\newcommand{\quadprojector}{{\rm Quad}(\projector)}

\newcommand{\Ared}{\widehat{A}}
\newcommand{\Bred}{\widehat{B}}
\newcommand{\Xred}{\widehat{X}}
\newcommand{\Lamred}{\widehat{\Lambda}}


\newcommand{\mycomment}{{\it Comments:}\ \ }

\newcommand{\DIAG}[2]{
\left(
\begin{array}{c c c c}
{#1}_1 & & & \\
 & {#1}_2 & & \\
 & & \ddots & \\
 & & & {#1}_{#2} 
\end{array}
\right)
}

\newcommand{\FDIAG}[3]{
\left(
\begin{array}{c c c c}
{#1}({#2}_1) & & &  \\
 & {#1}({#2}_2) & & \\
 & & \ddots &       \\
 & & & {#1}({#2}_{#3}) 
\end{array}
\right)
}

\newcommand{\Span}{{\rm span}}


\newcommand{\samp}{{\cal S}}
\newcommand{\period}{{\cal P}}
\newcommand{\cI}{{\cal I}}
\newcommand{\cIp}{{{\cal I}'}}
\newcommand{\computed}{({\rm comp})}
\newcommand{\round}{({\rm rnd})}
\newcommand{\truncate}{({\rm trunc})}
\newcommand{\alias}{({\rm alias})}


\newcommand{\iit}{\iitT\ }
\newcommand{\pit}{\pitT\ }
\newcommand{\iitT}{{\small IIT}}
\newcommand{\pitT}{{\small PIT}}

\newcommand{\opair}[2]{{(\{{#1}\}, {#2})}}

\newcommand{\translate}[1]{{\cal T}_{#1}}
\newcommand{\dilation}[1]{{\cal D}_{#1}}
\newcommand{\phaseshift}[1]{\Phi_{#1}}
\newcommand{\convolve}[2]{{#1}\,\conv\,{#2}}
\newcommand{\modulate}[2]{{#1}\,\cdot\,{#2}}
\newcommand{\sampling}[2]{{\cal S}\left({#1};\,{#2}\right)}
\newcommand{\periodize}[2]{{\cal P}\left({#1};\,{#2}\right)}


\newcommand{\sprod}{{\times}}
\newcommand{\conv}{{\ast}}
\newcommand{\Supp}{{(p)}}
\newcommand{\Supq}{{(q)}}

\newcommand{\dft}{{\rm DFT}}
\newcommand{\dftof}[1]{{\rm DFT}_{{#1}}}
\newcommand{\idft}[1]{{1\over {#1}}\overline{{\rm DFT}}_{{#1}}}

\newcommand{\cft}{{\cal F}}
\newcommand{\icft}{{\cal F}^{-1}}
\newcommand{\eye}{{\iota}}
\newcommand{\vgreek}[2]{{\left[ \matrix{{#1}_0 \cr {#1}_1 \cr \vdots \cr
                                        {#1}_{{#2}-1}\cr} \right]}}
\newcommand{\valphaN}{{\vgreek{\alpha}{N}}}
\newcommand{\vbetaN}{{\vgreek{\beta}{N}}}

\newcommand{\Mmu}{{M'}}

\newcommand{\Char}{\Gamma}
\newcommand{\bydef}{\stackrel{\mathrm{def}}{=}}

\newcommand{\Mplus}{{M^+}}
\newcommand{\support}{{\rm supp}}


\newcommand{\ftilde}{\tilde{f}}
\newcommand{\Ftilde}{\tilde{F}}
\newcommand{\alphatilde}{\tilde{\alpha}}
\newcommand{\betatilde}{\tilde{\beta}}
\newcommand{\band}{{\nu}}

\newcommand{\Indent}{\hspace*{0.2in}}




==> SupportDoc2/snn_macros.tex <==


\newcommand{\signature}{
\VS
Sincerely,\\
Ping Tak Peter Tang\\
Corresponding Author
}

\newcommand{\myfig}[5]{
\framebox[\textwidth]{
\epsfig{width=#2,height=#3,file=#1}
}
\caption{#4}\label{figure:#5}}

\newcommand{\PlaceHolder}[1]{
\framebox[0.9\textwidth]{
\parbox{0.4\textwidth}{
\begin{center}
{#1}
\end{center}}
}}

%\newcommand{\myfig}[4]{
%\framebox[6in]{
%\includegraphics{#1.#2}}
%\caption{#4}\label{figure:#3}}



\newtheorem{mydef}{Definition}
\newtheorem{mythm}{Theorem}
\newtheorem{myalgo}{Algorithm}
\newtheorem{mylemma}{Lemma}
\newtheorem{mycor}{Corollary}
\newtheorem{myprop}{Proposition}
\newtheorem{myassumption}{Assumption}
\newtheorem*{myproof}{Proof}


\newcommand{\placeholder}{{\small\bf PLACE HOLDER}}

\newcommand{\NI}{\noindent}
\newcommand{\VS}{{\vspace*{0.1in}\NI}}


\newcommand{\reals}{\mathbb{R}}
\newcommand{\complex}{\mathbb{C}}
\newcommand{\realpart}{\operatorname{Re}}
\newcommand{\suchthat}{\,\mid\,}
\newcommand{\equivto}{\Leftrightarrow}



\newcommand{\Bnorm}[1]{\| {#1} \|_B}
\newcommand{\Enorm}[1]{\| {#1} \|_2}
\newcommand{\Enormsq}[1]{\| {#1} \|_2^2}
\newcommand{\Onenorm}[1]{\| {#1} \|_1}
\newcommand{\inverse}[1]{{#1}^{-1}}
\newcommand{\transpose}[1]{{#1}^{\rm t}}
\newcommand{\dist}[2]{\mathrm{dist}({#1},{#2})}
\newcommand{\ssup}[2]{{#1}^{(#2)}}
\newcommand{\start}[1]{\ssup{#1}{0}}
\newcommand{\conv}{\ast}


\newcommand{\curr}{\mu}
\newcommand{\inputcurr}{b}
\newcommand{\currbias}{\lambda}
\newcommand{\poten}{v}
\newcommand{\potenthres}{\nu}
\newcommand{\spike}{\delta}
\newcommand{\spiketrain}{\sigma}
\newcommand{\avgcurr}{u}
\newcommand{\spikerate}{a}
\newcommand{\spiketime}[2]{t_{#1,#2}}
\newcommand{\decay}{\alpha}
\newcommand{\expwidth}{\tau}
\newcommand{\expdecay}[1]{e^{-{#1}/\expwidth}}
\newcommand{\dirac}{\delta}
\newcommand{\spt}[2]{t_{#1,#2}}


\newcommand{\vv}[1]{\mathbf{#1}}
\newcommand{\vd}[1]{\dot{\mathbf{#1}}}
\newcommand{\vva}{\vv{a}}
\newcommand{\vvb}{\vv{b}}
\newcommand{\vve}{\vv{e}}
\newcommand{\vvf}{\vv{f}}
\newcommand{\vvg}{\vv{g}}
\newcommand{\vvq}{\vv{q}}
\newcommand{\vvm}{\vv{m}}
\newcommand{\vvs}{\vv{s}}
\newcommand{\vvu}{\vv{u}}
\newcommand{\vvv}{\vv{v}}
\newcommand{\vvw}{\vv{w}}
\newcommand{\vvx}{\vv{x}}
\newcommand{\vvy}{\vv{y}}
\newcommand{\vvz}{\vv{z}}
\newcommand{\vvzero}{\vv{0}}


\newcommand{\cc}[1]{{\cal #1}}
\newcommand{\ccA}{\cc{A}}
\newcommand{\ccB}{\cc{B}}
\newcommand{\ccC}{\cc{C}}
\newcommand{\ccD}{\cc{D}}
\newcommand{\ccE}{\cc{E}}
\newcommand{\ccF}{\cc{F}}
\newcommand{\ccI}{\cc{I}}
\newcommand{\ccL}{\cc{L}}
\newcommand{\ccM}{\cc{M}}
\newcommand{\ccS}{\cc{S}}
\newcommand{\ccX}{\cc{X}}



\newcommand{\vvastar}{\vva^*}
\newcommand{\vvustar}{\vvu^*}
\newcommand{\ustar}{u^*}
\newcommand{\astar}{a^*}

\newcommand{\thresfun}{T}
\newcommand{\thres}{\thresfun_\lambda}
\newcommand{\vvthres}{\vv{\thresfun}_\lambda}
\newcommand{\lyap}{\xi}

\newcommand{\vvphi}{{\boldsymbol\phi}}

\newcommand{\vvT}{\vv{T}}
\newcommand{\vvF}{\vv{F}}

\newcommand{\vdu}{\vd{u}}

\newcommand{\ustart}{\ssup{\vv{u}}{0}}
\newcommand{\vstart}{\ssup{\vv{v}}{0}}
\newcommand{\vvahat}{\hat{\vva}}
\newcommand{\vvuhat}{\hat{\vvu}}
\newcommand{\vvvhat}{\hat{\vvv}}



\newcommand{\flowlasso}[2]{\vv{A}({#1},{#2})}
\newcommand{\flowlca}[2]{\vv{U}({#1},{#2})}
\newcommand{\vdA}{\vd{A}}
\newcommand{\vdU}{\vd{U}}

\newcommand{\grad}{\nabla}
\newcommand{\sign}{\mathrm{sign}}


\newcommand{\fixedpts}{{\cal F}}
\newcommand{\criticalpts}{{\cal C}}
\newcommand{\fixedregion}{\hat{\fixedpts}}




\newcommand{\ctrans}[1]{{#1}^{*}}
\newcommand{\tendsto}{\rightarrow}
\newcommand{\Chi}{\Pi}
\newcommand{\diag}{{\rm diag}}
\newcommand{\rank}{{\rm rank}}
\newcommand{\spann}{{\rm span}}
\newcommand{\gap}{{\rm gap}}
\newcommand{\offdiag}{{\rm off}}
\newcommand{\half}{\frac{1}{2}}
\newcommand{\tmpa}{{\rm dummy}}
\newcommand{\tmpb}{{\rm dummy}}
\newcommand{\tmpc}{{\rm dummy}}
\newcommand{\tmpd}{{\rm dummy}}

\newcommand{\Deltop}{\xi}
\newcommand{\Delbot}{\zeta}
\newcommand{\Deldc}{\psi}
\newcommand{\Deltrans}[1]{
\left[
\begin{array}{c | c}
  \begin{array}{c}
  \iterate{\Deltop}{#1} \\ 
  \iterate{\Delbot}{#1}
  \end{array}
 & \iterate{\Deldc}{#1}
\end{array}
\right]
}
\newcommand{\Linv}[1]{\iterate{L^{-1}}{{#1}}}


\newcommand{\quadf}{\rho}
\newcommand{\quadfbdd}{\xi}
\newcommand{\reference}{{\rm ref}}
\newcommand{\mm}{m}
\newcommand{\mprime}{m'}
\newcommand{\pp}{p}
\newcommand{\gapfactor}{\gamma}
\newcommand{\lambdamin}{\lambda_{-}}
\newcommand{\lambdamax}{\lambda_{+}}
\newcommand{\lambint}{(\lambdamin,\lambdamax)}
\newcommand{\lambintc}{[\lambdamin,\lambdamax]}
%\newcommand{\lambnum}{{\mathbf{i}}}
\newcommand{\lambnum}{e}
\newcommand{\surM}{M}
\newcommand{\calI}{{\cal I}}
\newcommand{\calC}{{\cal C}}
\newcommand{\projector}{{X_\calI}\ctrans{X}_\calI B}
\newcommand{\quadprojector}{{\rm Quad}(\projector)}

\newcommand{\Ared}{\widehat{A}}
\newcommand{\Bred}{\widehat{B}}
\newcommand{\Xred}{\widehat{X}}
\newcommand{\Lamred}{\widehat{\Lambda}}


\newcommand{\mycomment}{{\it Comments:}\ \ }

\newcommand{\DIAG}[2]{
\left(
\begin{array}{c c c c}
{#1}_1 & & & \\
 & {#1}_2 & & \\
 & & \ddots & \\
 & & & {#1}_{#2} 
\end{array}
\right)
}

\newcommand{\FDIAG}[3]{
\left(
\begin{array}{c c c c}
{#1}({#2}_1) & & &  \\
 & {#1}({#2}_2) & & \\
 & & \ddots &       \\
 & & & {#1}({#2}_{#3}) 
\end{array}
\right)
}

\newcommand{\Span}{{\rm span}}




\newcommand{\bydef}{\stackrel{\mathrm{def}}{=}}


\newcommand{\Indent}{\hspace*{0.2in}}




==> illustration.tex <==
\section{Illustration}

The numerical example has input chosen as follows:
\begin{equation}
\vvs = 
\begin{bmatrix}
0.5\\ 
1\\ 
1.5
\end{bmatrix}
,\: 
\Phi =
\begin{bmatrix}
0.3313 & 0.8148 & 0.4364 \\ 
0.8835 & 0.3621 & 0.2182 \\ 
0.3313 & 0.4527 & 0.8729
\end{bmatrix}
\end{equation}

\noindent and $\lambda=0.1$.




==> intro.tex <==
\section{Introduction}

A central question in computational neuroscience is to understand how complex
computations emerge from networks of neurons.
Many computation models have been proposed to solve various information processing
problems.
For example, certain optimization problems can be solved with Hopfield network,
and function approximation can be performed using artificial neural networks.
These models have also inspired the development of parallel computation algorithms
and architecture to exploit the inherent parallelism in neuron models.
The neurons in these models, however, have major gaps to being biologically realistic.
In particular, conventional computational models often assume neurons can exchange 
analog state variables. 
Real biological neurons communicate with each other using discrete spike trains. 
However, it is unclear how this communication of analog state information 
can be realized efficiently with spiking neurons.

Recent progress in optimality-driven balanced network sheds lights on this problem \cite{deneve2016efficient}.
It is argued that in a tightly balanced excitatory/inhibitory network,
spikes occur from a competitive process between neurons,
and serve to minimize a network-level energy function.
Neuron communication in this framework is highly efficient with spikes.
Instead of encoding analog values as spike rates,
each spike is precisely timed to keep the network in optimality.
This line of work, however, mostly focus on network behaviors at the
steady-state (i.e., when the optimality is reached) such as \cite{boerlin2013predictive}.
The convergence of such networks has not yet been analyzed nor fully studied.

In this work, we provide a framework to rigorously establish the convergence of firing
rates in a spiking neural network.to solutions corresponding to a LASSO problem.
This network model, namely the Spiking LCA, is first proposed in \cite{shapero2013configurable} to implement
the LCA algorithm \cite{rozell2008sparse} (we will call this the Analog LCA for clarity) using
integrate-and-fire neurons in analog circuit.
The convergence is established in two stages.
First, the convergence of Analog LCA to LASSO is established using a generalization
of LaSalle's invariance principle.
The convergence result can be applied to a non-negative variant of Analog LCA,
which is important in the context of spiking neurons where firing rates can never be negative.
Second, we show that under a particular firing rate formulation,
the firing rates in Spiking LCA converge to the fixed point in the corresponding Analog LCA.
This convergence emerges from a moderate assumption that the inter-spike intervals 
cannot be arbitrarily long unless the neuron stops spiking.

Finally, we provide numerical simulations to demonstrate convergence
in large-scale spiking neural networks.
Interestingly, the network only needs very few spikes between neurons before it converges.
It is observed that the convergence of Spiking LCA is not slower than Analog LCA,
but with much fewer communication between neurons.
Due to the reduced communication cost, our numerical implementation of Spiking LCA
can even be competitive in execution time comparing to the fastest LASSO solver such as FISTA,
at the cost of a reduced numerical precision in the solution.
This opens up an avenue for future algorithm design and computer architecture research.


